CRASH: Challenging Reinforcement-Learning Based Adversarial Scenarios For Safety Hardening

Ensuring the safety of autonomous vehicles (AVs) requires identifying rare but critical failure cases that on-road testing alone cannot discover. High-fidelity simulations provide a scalable alternative, but automatically generating realistic and diverse traffic scenarios that can effectively stress test AV motion planners remains a key challenge. This paper introduces CRASH - Challenging Reinforcement-learning based Adversarial scenarios for Safety Hardening - an adversarial deep reinforcement learning framework to address this issue. First CRASH can control adversarial Non Player Character (NPC) agents in an AV simulator to automatically induce collisions with the Ego vehicle, falsifying its motion planner. We also propose a novel approach, that we term safety hardening, which iteratively refines the motion planner by simulating improvement scenarios against adversarial agents, leveraging the failure cases to strengthen the AV stack. CRASH is evaluated on a simplified two-lane highway scenario, demonstrating its ability to falsify both rule-based and learning-based planners with collision rates exceeding 90%. Additionally, safety hardening reduces the Ego vehicle's collision rate by 26%. While preliminary, these results highlight RL-based safety hardening as a promising approach for scenario-driven simulation testing for autonomous vehicles.

==> contributions.tex <==

In this work we developed methods that can automatically falsify the motion planner for an autonomous vehicle in simulation, and then improve the motion planner to be robust against the generated falsification. Our contributions are as follows:

\begin{enumerate}
    \item Firstly, we use reinforcement learning to control an adversarial agent to automatically falsify a rule-based and learning-based motion planner in simulation.
    \item We formalize the problem of safety hardening, where we close the loop and improve the learning-based planner by retraining it against the adversarial agent. We use a technique termed safety hardening to iteratively retrain both the adversarial agent and the Ego vehicle, continuously exposing the Ego against stronger adversarial agents. To decide which adversarial agents and Ego vehicles to train each other against, we developed two variants of safety hardening using local and model-pool based methodologies. Within the model-pool methods we tested multiple sampling strategies; uniform and weighted sampling, scoring agents using Elo to properly weight them. To score agents fairly we use periodic round-robin style tournaments.
\end{enumerate}

In addition to the above contributions, we explored several future research directions within the context of this problem. We discuss incorporating the behavioral intent of other vehicles and a prediction of their future motion, as well as accounting for the inherent asymmetry in fairly scoring agents.


==> discussion.tex <==
Exploring the behavior of agents in longer cycles with many tunable parameters in the DQN, Elo computation, and tournament evaluations proved to cause slow and manual analysis. There is inherent unfairness in the Elo evaluation between the Ego and NPC, and we discuss the reasoning behind this claim.
In addition, to further explore the different effects of Elo and Tournaments on Safety Hardening, we reduced the complexity of the problem further to only the behind left scenario, $S_0^{BL}$ and kept a maximum of two cycles. 
With the simplified setting, we explored some nuances in our problem setting that show potential for further research.

\subsection{Scenario Asymmetry}


For each game between an Ego and NPC, there is an inherent unfairness in their Elo evaluation. In the adjacent scenarios $S_{0}^{AR,AL}$, the NPC can make an immediate lane change to cause a collision in one time step, rendering it impossible for the Ego to avoid collision no matter what. The Elo 


While we rate both the Ego and NPC vehicle with the same Elo equation, and their update functions are identical to each other. However, the scenario for both vehicles is not symmetric, where the NPC can have an easier time causing a collision with the Ego in the $S_0^{AL}$ and $S_0^{AR}$ states. A trained NPC vehicle can cause a collision with the Ego in one time step if it immediately performs a lane change maneuver, shown in Figure~\ref{fig:scenariocrashrate}, compared to the far longer trajectories shown in Figure~\ref{fig:training_history}. Equation~\ref{eq:ego_rating_update} defines the Elo rating update for each agent, where the parameter $K$ acts as a gain factor determining the magnitude of the rating adjustment based on the outcome of an episode. Utilizing a constant $K$ value for all episodes implies that each episode outcome is equally significant in assessing an agent's skill level.

When introducing multiple starting configurations into each episode, it becomes evident that certain scenarios inherently favor the NPC in causing collisions, while others do not. Specifically, in the adjacent left/right scenarios, once the NPC learns to execute a rapid lane change, it becomes nearly impossible for the Ego agent to avoid a collision. 


In the domain of chess, higher-ranked players have their ratings updated using a reduced $K$ value, resulting in less variance in their rating adjustments~\cite{Elo1967}. Inspired by this approach, we propose to adjust the gain for the Elo update based on the starting state of each episode. For adjacent scenarios, we can set $K = 8$, while for the other scenarios, we use $K = 32$, the standard update value for chess. This modification aims to normalize the Elo updates such that NPC agents do not receive disproportionately large Elo increases for causing collisions in the adjacent scenarios, and Ego agents do not suffer excessive Elo losses.


\subsection{Ego behavior in Behind Left Scenario}

During examination of the tournament evaluation, we noticed that when seeding the episodes with only behind left, $S_{0}^{BL}$, the NPC vehicle would not be able to falsify the Ego vehicle or cause any crashes. When the NPC is spawned behind left, it has to speed up to catch up to the Ego and cause a collision. The Ego vehicle was incentivized to always speed up to the maximum velocity, making it impossible for the NPC to catchup. The collision avoidance reward signal in Eq. \ref{eq:ego_reward} which is the default reward in highway-env, lacked a reduction of reward when the Ego vehicle exceeded the max velocity.

This problem led to the exploration of how the trained agents behave when there is no adversarial agent. The introduction of NPC agents, should not cause the Ego agent to drive unrealistically, but that was not observable in the behind left scenario due to the Ego vehicles speed incentive.

Altering the reward function to reduce reward when exceeding the maximum speed and reducing the speed range to $[20, 20.5]$ resulted in the Ego vehicle maintaining speed and when exposed to a NPC agent it would speed up.

\subsection{Behavior Prediction}
\label{sec:behavior_prediction}

\begin{figure}[t]
\centering
    \includegraphics[width=\linewidth]{figures/state10_state11_speed_sr.pdf}
    \caption{Ego Speed and Crash Rate when trained against a MOBIL and NPC agents. In the top left plot, the Ego Speed vs MOBIL is shown and the Crash rate is in the bottom left. While the crash rate stays low, using the augmented state vector the Ego doesn't unnecessarily speed up against the MOBIL agent. In the top right plot, the Ego Speed vs the NPC is shown, and the Crash rate is in the bottom right. The augmented state vector helps the Ego speed up against the NPC faster than it does against MOBIL, as well as reducing the overall crash rate.}
    \label{fig:augmentedstate}
\end{figure}

When the Ego agent is trained against an adversarial NPC, they no longer maintain the velocity in the nominal speed range when evaluated against the original MOBIL agent. There is currently no state information that would inform the Ego agent about the intention of the other agent. In order to distinguish between an adversarial agent or a non adversarial one, the Ego would have to be able to predict the motion of the NPC.

The current training pipeline does not take into account any temporal aspect of state, or any history of motion of either vehicle. Prediction pipelines for autonomous driving can be setup by utilizing some form of memory such as LSTM networks or by gathering historical observations of the other agent. Usually, these types of pipelines are integrated into autonomous driving perception pipelines. Since the current scope of our research is to focus on motion planning, we would like to abstract away the need for predicting the intent of the other vehicle.

We augment the state of the Ego Vehicle, including a marker that indicates whether or not the NPC agent is a Adversarial DQN agent, or MOBIL. In the behind left scenario, we train an Ego agent for 1000000 transitions against a uniform sampling of $V_{1}$ as well as $E_{0}$, the MOBIL agent. We observe that the Ego will speed up unnecessarily against the MOBIL controlled NPC in Fig~\ref{fig:augmentedstate}. Against the NPC it also speeds up, but learns over time. When adding in our augmented state, the Ego vehicle no longer speeds up against the MOBIL agent, and learns to speed up against the NPC with a lower sample rate. Using this binary indicator the Ego is able to maintain the correct speed against both the MOBIL and NPC agents, while maintaining the same crash rate against MOBIL and a lower crash rate vs the NPC.

This supports the idea that the Ego agent needs to predict the behavior of the NPC in order to properly deal with adversarial scenarios while maintaining the ability to drive in normal traffic, and we will perform future experiments with longer cycles and 

==> future_work.tex <==
Our initial implementation of Safety Hardening, shows a rich problem space in which to further explore this research. We can identify several research questions to push this work further. 

\begin{enumerate}
    \item Can different reinforcement learning methodologies improve the change in crash rate for falsification and hardening?
    \item Can we generate more realistic falsifications by trying to cause collisions that place the Ego at fault?
    \item Can we generate more complex falsifications by scaling safety hardening with more NPCs and different road geometries?
\end{enumerate}

 All of these directions seek to improve the saliency and realism  of the generated trajectories in simulation.


\begin{figure}
    \centering
     \includegraphics[width=0.8\linewidth]{figures/ablationstudy.png}
     \caption{Proposed ablation study over Reinforcement Learning algorithm type and Neural Network hyperparameters.}
     \label{fig:ablation_study}
 \end{figure}

\subsection{DQN Parameter Ablation Study}
\label{sec:AblationStudy}

Many of the parameters in the initial DQN implementation were chosen arbitrarily, or used as default values for DQNs applied toward Atari games. We will provide a quantitative analysis of these parameters by doing an ablation study, specifically on the various types of replay memory buffers (size and prioritization), DQN hyperparameters (discount factor, hidden dimension size, target update rate), and $\epsilon$ greedy action selection parameters ($\epsilon_{start}, \epsilon_{end}, \epsilon_{decay}$).

We would also like to explore other reinforcement learning algorithms for discrete action selection, such as Soft-Actor-Critic \cite{haarnoja2018soft} and Proximal Policy Optimization \cite{schulman2017proximal} methods. This would require extending the ablation study to the parameters required by these algorithms as well. Overall we will explore the different algorithm structures shown in Figure \ref{fig:ablation_study}. 

\subsection{Collision Specific Reward Functions}
\label{sec:CollisionSpecificReward}

In our preliminary findings detailed in Section~\ref{sec:FalsificationResults}, the most predominant types of crashes were aggressive side swipes and rear-end collisions, as illustrated in Fig~\ref{fig:collision_example}. Notably, the CA DMV Disengagement Reports for Autonomous Vehicles, which we previously referenced, delineate up to 8 distinct collision types pertaining to vehicles. This report provides an even more nuanced breakdown of vehicle damage, as showcased in Fig~\ref{fig:collision_report}. To further refine our approach, we will modify the collision reward, $r_c$, so that it is granted only when the observed trajectory meets a predetermined geometric criterion.

By training an agent on specific collision types, we hope to achieve a higher level of granularity and realism in simulations. This granularity allows for more realistic testing scenarios, ensuring that autonomous vehicles are tested against a diverse range of potential collision situations rather than just generic or random ones. Understanding specific types of collisions can help in identifying weaknesses or vulnerabilities in the autonomous vehicle's motion planner. If a particular type of collision is more prevalent, it may indicate a specific flaw or oversight in the autonomous system that needs addressing.

Therefore we plan to train our reinforcement learning agent to collide with the autonomous vehicle, with respect to each of the disengagement report collision types. We can define the NPC's collision with the Ego vehicle as a geometric problem  that emulates these collision types, and design reward functions to learn the trajectory required to collide with the Ego as specified.

We will need to (1) define a taxonomy of collision types, classifying the collision type (side-swipe, rear-end, etc.) of each trajectory. With specific collision types defined we will then (2) design new reward functions that lead towards learning how to generate these trajectories that lead to the specific collision types.

\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
    \includegraphics[width=\linewidth]{figures/specific_collisions.png}
    \caption{Collision Types observed during DQN training}
    \label{fig:collision_example}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
     \includegraphics[width=\linewidth]{figures/Screenshot from 2023-07-22 12-42-14.png}
     \caption{Collision Report Damaged Area}
     \label{fig:collision_report}
\end{subfigure}  
\caption{Specific types of collision scenarios that we want our specific reward fucntions to encourage.}
\end{figure}

\subsection{Multiple Adversarial NPCs}
\label{sec:MultiAgent}

As autonomous driving systems progress, they must be able to interact with multiple dynamic entities in the environment simultaneously. Our analysis of specific collision trajectories is driven by the goal of making these trajectories more realistic and complex. In tandem to this goal, we will add more NPC vehicles to the simulation and have our policy control multiple NPC vehicles. 
By having multiple NPCs in our simulations, we can simulate more realistic driving scenarios. This offers a closer approximation to real-world situations where the autonomous vehicle will interact with multiple vehicles.
Implementing multi-agent systems might introduce new challenges related to computational efficiency and policy convergence. We'll need to adapt our training protocols to ensure scalability and robust learning across all agents.
While using a single policy to control multiple NPCs offers the advantage of a unified strategy, it might be too generalized for specific NPCs’ needs. On the other hand, employing separate asynchronous policies for each NPC provides the flexibility of tailoring actions to each NPC's unique situation but can lead to less coordinated behavior.

Deciding how to incorporate multiple agents into safety hardening and our agent ranking is also an interesting problem space. Coordinating NPCs may be more successful in causing collisions, and can be ranked higher than non coordinated NPCs. Exploring whether to rank NPCs as individual agents or as teams of agents. 

After deciding on a multi agent approach, we will alter the collision specific reward function to encourage the NPCs to collide with the Ego vehicle, and not with each other. The difference between using a single multi-agent policy or multiple policies can be seen in Figure \ref{fig:multi-agent-goal}.


\begin{figure}
    \centering
     \includegraphics[width=0.8\linewidth]{figures/multi-agent-and-scaling.png}
     \caption{We want to scale the collision problem to encompass more diverse driving scenarios, with multiple controllable adversarial NPCs. This will involve exploring different types of multi-agent control policies.}
     \label{fig:multi-agent-goal}
 \end{figure}
 
\subsection{Learning the Initial Configuration}
\label{sec:LearningInitialConfig}


In each simulator reset, the environment starting state is chosen from a set of predefined configurations. This is done in order to vary the starting trajectories such that the policy will not overfit to a specific starting state.

Our initial set of possible states based on the two lane highway is quite small, and thus it is possible to enumerate the different states. If we use a more complex and realistic road geometry such as an intersection, roundabout, or multiple lane highway, the initial state space will grow dramatically. Manually enumerating the different starting states will not be realistic anymore and we will have to explore methodologies to determine how to spawn the initial agents.

Additionally, while predefined configurations provide variety, they might not always offer the most challenging or relevant scenarios for our policy's goals. Hence, there's a need to dynamically determine the most useful starting states. Our hypothesis is that certain configurations may be more conducive to revealing vulnerabilities in the policy or leading to novel collision trajectories.

How do we determine what configuration to examine? Which starting state is most useful to observe in order to quickly generate novel collision trajectories?
To address this, we propose an auxiliary policy that learns to select the initial configuration settings for the simulator. The aim is for this policy to prioritize configurations that have historically led to new and intriguing trajectories or those that present more challenging scenarios for the learning agent. By allowing the system to learn and decide its starting state, we introduce an adaptive component that pushes the boundaries of the agent's learning. This ensures that as the agent becomes proficient in one scenario, it's continually presented with newer challenges, leading to a more comprehensive understanding of potential collision trajectories.

An initial approach for this problem would be to learn a policy to generate the initial states of the Ego and NPC vehicles. Further exploration of this problem could lead to a hierarchical approach as well, where a high level policy determines the initial starting state, and a lower level policy controls the NPC actions.

\begin{figure}
     \includegraphics[trim={0 0 0 0.9cm},clip,width=\linewidth]{figures/research_goal_4.pdf}
     \caption{Rather than resetting the simulator to a state $S_{0}$ within the predefined set of starting states $C$, we want to learn the starting states $S_{0}$ that initializes the simulator.}
     \label{fig:rg4}
 \end{figure}


==> introduction.tex <==
Research in Autonomous Vehicles (AV) has exploded since the DARPA Grand Challenge in 2004, but after two decades of continuous research and substantial industry involvement, deploying safe and reliable self-driving cars is still an unsolved problem. Remarkable progress has been made in the domain, where companies such as Waymo, Cruise, and Tesla to name a few, are testing AVs as robotaxis, and are able to demonstrate short term success in increasing driving safety \cite{Kusano2023ComparisonOW}. 
However, fully autonomous vehicles as described in the Society of Automotive Engineers (SAE) Levels 0-5 standard \cite{SAEJ3016_2021}, is still an unreached goal. AV software stacks are a complex combination of rule-based and learning-based components handling perception, motion planning, and control, where failures in any one component can have cascading effects and cause potential collisions. 
Despite this, AVs are being deployed and tested on road at an increasingly rapid rate \cite{AP2023, Muller2023}, without safety driver systems in multiple new cities simultaneously. 

In San Francisco and Phoenix, where the majority of these AV systems are tested, several high profile incidents have occurred that do not incur confidence or transparency in AV operation. The most prominent example is Cruise dragging a pedestrian after they were struck by another vehicle and their subsequent withholding of information to government officials \cite{Exponent2024CruiseReport}, leading to the revocation of their license to carry passengers. 
Waymo and Zoox are under federal investigation due to the numerous traffic violations and erratic driving behavior, resulting in several crashes \cite{NHTSA2024WaymoInvestigation, NHTSA2024ZooxInvestigation}. 
Regardless of accident fault, there is little to no public disclosure for the reason behind these accidents.
Commercial robotaxis are black boxes where insight into their operations and failures are kept inhouse.
Visibility into AV accidents is limited to the California Department of Motor Vehicles (CA DMV) crash and disengagement reports \cite{Team2021}, as well as the National Highway Traffic Safety Adminstration (NHTSA) standing order on reporting autonomous vehicle crashes \cite{NHTSA2024ADSReport12345}. 
The disengagement reports provide details about the company operating the vehicle, whether it was autonomous or not, and a cursory overview of the incident. The crash reports from CA DMV try to provide more detail and a description of the crash and damage, but there is no discussion of any of the autonomous system components.
These reports are collected by mandatory self-reporting and are attempts at objective description of the situation, but sometimes high profile accidents are not reported to the database, making it both an incomplete and biased representation of accidents. 
Since there is little to no insight into the reasoning behind the AV's decision making, this can lead to unresolved accountability of the situation \cite{Vang2023}. 

These reoccurring accidents and their associated reports clearly indicate that current AV technology is not robust to edge cases and unfamiliar situations.
They are examples of real-world falsification, where in the context of autonomous vehicles, 'falsification' refers to scenarios that cause system failures.
Each scenario encompasses all the elements—traffic lights, pedestrians, vehicles, road rules, and navigation goals—that an AV would encounter in real-world conditions. 
Several open source AVs succeed in most common driving scenarios \cite{li2024rigoroussimulationbasedtestingautonomous}, but in uncommon and rare situations cautionary situations and even failures can occur.
AV software stacks may have only been designed for specific operating conditions such as geofenced areas \cite{Hardigree2023}, but when venturing outside of those constraints the reliability of the system comes into question. 
Even within the constraints set by the AV design, the variability in these areas is large enough that on road testing alone is not enough to discover all possible dangerous or relevant scenarios \cite{hasuo_responsibility-sensitive_2022}.
To establish a statistical guarantee of safety is impractical, as the billions of miles required to drive by the AVs to validate an increased performance margin over human drivers will take an astronomical amount of time \cite{hasuo_responsibility-sensitive_2022}. 
Consequently, alternatives to real-world driving need to be explored to expedite this validation process.

Simulation is a useful tool to repeatedly run driving scenarios, and iteratively test the AV's perception, planning, and control systems.
As such, it is a useful tool in searching for rare situations where the AV might fail within a particular driving scenario, such as an intersection or dealing with 
The importance of testing these systems in simulation is crucial to the exploration of untested scenarios for the autonomous system, as well as the speed of testing.  
Numerous autonomous vehicle companies use extensive simulation to validate their safety systems, examples being Waymo's CarCraft \cite{Waymo2021}, NVIDIA's DriveSim \cite{NVIDIAConstellation}, and Waabi World \cite{WaabiWorld}.


Relying solely on onroad testing is (1) a threat to public safety, using a city with pedestrians and other drivers as a testing environment. (2) Discovering edge cases in the real world, leads to slow iteration of testing, as it will take an increasingly long time to discover unforeseen situations. Testing within simulation allows the AV to encounter a potentially dangerous situation and assess it's capability in a safe environment, but which scenarios should we test the simulated AV with? Simply waiting for the simulation to encounter rare tail-end scenarios lends itself to the same inefficiency in manual analysis of real world testing. 


\subsection{Challenges with AV Simulation}
Scenario generation for simulation poses three main challenges, of saliency, dimensionality, and rarity. 

\begin{enumerate}
    \item{\textbf{Saliency:}}
    A generated scenario should be realistic and relevant for the purposes of testing.
    Ensuring the dynamics of the simulation represent real physical systems ensures that unrealistic steering maneuvers or acceleration capabilities do not obfuscate evaluating the efficacy of the AV stack. 
    Also ensuring the realism of the scenario itself, is important to ensure the scenario being tested would actually be encountered in the real world.
    At the same time, repeatedly testing traffic scenarios where the other vehicles or dynamic conditions don't effectively test the AV is not a useful simulation criterion.
    \item{\textbf{Dimensionality:}}
    The second challenge of simulation is the high dimensionality of the autonomous vehicle scenario. 
    For every axes on which the simulation can be varied, such as the number of vehicles, how they are arranged, the behavior of these vehicles the number of scenarios to examine increases exponentially. 
    This grows in scope wildly as pedestrians, cyclists, traffic rules, road infrastructure, navigation goals, are all introduced as decision variables in just how to initialize the simulation environment. 
    This "curse of dimensionality" presents the question of what should we even begin to examine?
    \item{\textbf{Rarity:}}
    The third challenge, is the "curse of rarity" where within this vast spectrum of scenarios, there exists a small number of useful scenarios that will test or reveal relevant weaknesses in the AV. Real world driving shows that there is a fatality rate of 1 person per 100 million miles driven, \cite{nhtsaFatalityAnalysis}. 
    To achieve this metric for autonomous vehicles as well and possess the same statistical guarantee as human drivers, these systems would need to be driven for billions of miles. 
    The term "long tail" is borrowed from statistics and describes the phenomenon where certain scenarios occur with very low frequency but are crucial for comprehensive testing.
    Frequent descriptions of scenario simulation describe "long tail" scenario generation \cite{zhou2022longtail}, referring to the tail end of a scenario distribution. 
    This tail end represents situations that the autonomous system might only encounter once in several million or even billion miles of driving. 
    However, despite their rarity, these "long tail" events can pose significant challenges for AV systems due to their unpredictability and potential for hazardous outcomes.
    It's these uncommon scenarios that, while infrequent, might lead to unexpected system behaviors, making their identification and simulation vital for ensuring the safety and reliability of autonomous vehicles.
\end{enumerate}


Rare and realistic and scenarios are desirable simulation targets; it is assumed that any potential AV failures will lie in these unseen and untested situations..
For example, the situation with Cruise dragging a pedestrian is an excellent example of a rare scenario, or edge case.
Handling the situation of what to do in a post-collision situation beyond just slowing down and moving to the side of the road, may not fall under the purview of most AV testing pipelines.

Testing the above edge case in simulation before encountering them on the road is the ideal situation, but defining every rare situation is not feasible.

Traditional methods of AV validation involve waiting to encounter rare or unexpected conditions in on-road tests or simulations. 
This passive approach can be time-consuming and, due to its reactive nature, might not cover the exhaustive range of potential edge cases. 
The challenge then becomes identifying an approach that can actively probe the system's vulnerabilities. 
Actively seeking out potential failure modes allows for a more systematic understanding of system weaknesses and avenues for refinement.

\subsection{Goals of Research}

The goal of our research is to automatically falsify the AV, then subsequently close the loop and robustify the AV against the falsification. Falsification can apply to any part of the AV stack, whether it be perception, planning, or control. In many of the CA DMV disengagement reports, the autonomy component reported as failing is the perception system, which can cause downstream failures in planning, and then control. Perception systems have their own intricate sensor pipelines where there are numerous attack vectors on causing LiDAR, camera, or radar systems to fail to report a detection \cite{guesmi2024navigatingthreatssurveyphysical, remoteperception2024, yao2024exploringradardatarepresentations}. For simplification, we assume that the AV perception system provides a seamless ground truth detection of the scenario's other vehicles, objects, and road details, and decide to focus on falsification of the motion planning module of the AV stack. Typically the perception pipeline of the AV provides a bounding box or grid-world style representation of other vehicles, which the AV motion planner will process to provide a collision free trajectory to follow \cite{Teng_2023}. Similarly, we seek to automatically generate scenarios where the AV motion planner will produce a trajectory that causes a collision. Then given the colliding trajectory, we will specifically improve the AV motion planner.

We assume that we can find these falsifications within rare and novel situations, and seek to use a methodology that can produce these rare trajectories. Deep Reinforcement Learning (DRL) has shown promise in producing novel behavior to solve Atari games, robotic manipulation, and other closed loop control tasks \cite{mnih2013playingatarideepreinforcement, tang2024deepreinforcementlearningrobotics}. We propose this method will be suitable for dynamically probing the vulnerabilities of the AV motion planner. Due to the highly nonlinear nature of AV motion planning, DRL's strengths in non-linear estimation and adaptive learning \cite{lillicrap2019continuous, mnih2015humanlevel} will prove a suitable candidate to generate the proposed falsification trajectories.  

Using DRL, we will directly generate motion planner trajectories that cause the AV to crash, and thus a falsification. Then using the same mechanism, we will refine the AV motion planner to avoid the colliding trajectory. We seek to perform the automatic falsification and subsequent improvement in an iterative fashion, until we produce both a an effective falsifier, and a more robust AV motion planner.


